Resolution of the $k$-Dirac operator

This is the second part in a series of two papers. The $k$-Dirac complex is a complex of differential operators which are natural to a particular $|2|$-graded parabolic geometry. In this paper we will consider the $k$-Dirac complex over a homogeneous space of the parabolic geometry and as a first result, we will prove that the $k$-Dirac complex is exact with formal power series at any fixed point. Then we will show that the $k$-Dirac complex descends from an affine subset of the homogeneous space to a complex of linear, constant coefficient differential operators and that the first operator in the descended complex is the $k$-Dirac operator studied in Clifford analysis. The main result of this paper is that the descended complex is locally exact and thus it forms a resolution of the $k$-Dirac operator.

==> young_diag_small.tex <==

\def\sYj{                  %1
\begin{picture}(3,3)
\put(0,3){\line(1,0){3}}
\put(0,0){\line(1,0){3}}
\put(0,3){\line(0,-1){3}}
\put(3,3){\line(0,-1){3}}
\end{picture}}


\def\sYjj{                 %11
\begin{picture}(3,6) 
\put(0,6){\line(1,0){3}}
\put(0,3){\line(1,0){3}}
\put(0,0){\line(1,0){3}}
\put(0,6){\line(0,-1){6}}
\put(3,6){\line(0,-1){6}}
\end{picture}
}



\def\sYjjj{                 %111
\begin{picture}(3,9) 
\put(0,9){\line(1,0){3}}
\put(0,6){\line(1,0){3}}
\put(0,3){\line(1,0){3}}
\put(0,0){\line(1,0){3}}
\put(0,9){\line(0,-1){9}}
\put(3,9){\line(0,-1){9}}
\end{picture}
}



\def\sYjjjj{                 %1111
\begin{picture}(3,12) 
\put(0,12){\line(1,0){3}}
\put(0,9){\line(1,0){3}}
\put(0,6){\line(1,0){3}}
\put(0,3){\line(1,0){3}}
\put(0,0){\line(1,0){3}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\end{picture}
}



\def\sYd{                 %2
\begin{picture}(6,3) 
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){6}}
\put(0,3){\line(0,-1){3}}
\put(3,3){\line(0,-1){3}}
\put(6,3){\line(0,-1){3}}
\end{picture}
}



\def\sYdj{                 %21
\begin{picture}(6,6) 
\put(0,6){\line(1,0){6}}
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){3}}
\put(0,6){\line(0,-1){6}}
\put(3,6){\line(0,-1){6}}
\put(6,6){\line(0,-1){3}}
\end{picture}
}



\def\sYdjj{                 %211
\begin{picture}(6,9) 
\put(0,9){\line(1,0){6}}
\put(0,6){\line(1,0){6}}
\put(0,3){\line(1,0){3}}
\put(0,0){\line(1,0){3}}
\put(0,9){\line(0,-1){9}}
\put(3,9){\line(0,-1){9}}
\put(6,9){\line(0,-1){3}}
\end{picture}
}



\def\sYdjjj{                 %2111
\begin{picture}(6,12) 
\put(0,12){\line(1,0){6}}
\put(0,9){\line(1,0){6}}
\put(0,6){\line(1,0){3}}
\put(0,3){\line(1,0){3}}
\put(0,0){\line(1,0){3}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){3}}
\end{picture}
}



\def\sYdd{                 %22
\begin{picture}(6,6) 
\put(0,6){\line(1,0){6}}
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){6}}
\put(0,6){\line(0,-1){6}}
\put(3,6){\line(0,-1){6}}
\put(6,6){\line(0,-1){6}}
\end{picture}
}



\def\sYddj{                 %221
\begin{picture}(6,9) 
\put(0,9){\line(1,0){6}}
\put(0,6){\line(1,0){6}}
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){3}}
\put(0,9){\line(0,-1){9}}
\put(3,9){\line(0,-1){9}}
\put(6,9){\line(0,-1){6}}
\end{picture}
}



\def\sYddjj{                 %2211
\begin{picture}(6,12) 
\put(0,12){\line(1,0){6}}
\put(0,9){\line(1,0){6}}
\put(0,6){\line(1,0){6}}
\put(0,3){\line(1,0){3}}
\put(0,0){\line(1,0){3}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){6}}
\end{picture}
}



\def\sYddd{                 %222
\begin{picture}(6,9) 
\put(0,9){\line(1,0){6}}
\put(0,6){\line(1,0){6}}
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){6}}
\put(0,9){\line(0,-1){9}}
\put(3,9){\line(0,-1){9}}
\put(6,9){\line(0,-1){9}}
\end{picture}
}



\def\sYdddj{                 %2221
\begin{picture}(6,12) 
\put(0,12){\line(1,0){6}}
\put(0,9){\line(1,0){6}}
\put(0,6){\line(1,0){6}}
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){3}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){9}}
\end{picture}
}



\def\sYdddd{                 %2222
\begin{picture}(6,12) 
\put(0,12){\line(1,0){6}}
\put(0,9){\line(1,0){6}}
\put(0,6){\line(1,0){6}}
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){6}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){12}}
\end{picture}
}



\def\sYt{                 %3
\begin{picture}(9,3) 
\put(0,3){\line(1,0){9}}
\put(0,0){\line(1,0){9}}
\put(0,3){\line(0,-1){3}}
\put(3,3){\line(0,-1){3}}
\put(6,3){\line(0,-1){3}}
\put(9,3){\line(0,-1){3}}
\end{picture}
}



\def\sYtj{                 %31
\begin{picture}(9,6) 
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){9}}
\put(0,0){\line(1,0){3}}
\put(0,6){\line(0,-1){6}}
\put(3,6){\line(0,-1){6}}
\put(6,6){\line(0,-1){3}}
\put(9,6){\line(0,-1){3}}
\end{picture}
}



\def\sYtjj{                 %311
\begin{picture}(9,9) 
\put(0,9){\line(1,0){9}}
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){3}}
\put(0,0){\line(1,0){3}}
\put(0,9){\line(0,-1){9}}
\put(3,9){\line(0,-1){9}}
\put(6,9){\line(0,-1){3}}
\put(9,9){\line(0,-1){3}}
\end{picture}
}


\def\sYtjjj{                 %3111
\begin{picture}(9,12) 
\put(0,12){\line(1,0){9}}
\put(0,9){\line(1,0){9}}
\put(0,6){\line(1,0){3}}
\put(0,3){\line(1,0){3}}
\put(0,0){\line(1,0){3}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){3}}
\put(9,12){\line(0,-1){3}}
\end{picture}
}



\def\sYtd{                 %32
\begin{picture}(9,6) 
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){9}}
\put(0,0){\line(1,0){6}}
\put(0,6){\line(0,-1){6}}
\put(3,6){\line(0,-1){6}}
\put(6,6){\line(0,-1){6}}
\put(9,6){\line(0,-1){3}}
\end{picture}
}



\def\sYtdj{                 %321
\begin{picture}(9,9) 
\put(0,9){\line(1,0){9}}
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){3}}
\put(0,9){\line(0,-1){9}}
\put(3,9){\line(0,-1){9}}
\put(6,9){\line(0,-1){6}}
\put(9,9){\line(0,-1){3}}
\end{picture}
}


\def\sYtdjj{                 %3211
\begin{picture}(9,12) 
\put(0,12){\line(1,0){9}}
\put(0,9){\line(1,0){9}}
\put(0,6){\line(1,0){6}}
\put(0,3){\line(1,0){3}}
\put(0,0){\line(1,0){3}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){6}}
\put(9,12){\line(0,-1){3}}
\end{picture}
}



\def\sYtdd{                 %322
\begin{picture}(9,9) 
\put(0,9){\line(1,0){9}}
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){6}}
\put(0,9){\line(0,-1){9}}
\put(3,9){\line(0,-1){9}}
\put(6,9){\line(0,-1){9}}
\put(9,9){\line(0,-1){3}}
\end{picture}
}


\def\sYtddj{                 %3221
\begin{picture}(9,12) 
\put(0,12){\line(1,0){9}}
\put(0,9){\line(1,0){9}}
\put(0,6){\line(1,0){6}}
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){3}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){9}}
\put(9,12){\line(0,-1){3}}
\end{picture}
}


\def\sYtddd{                 %3222
\begin{picture}(9,12) 
\put(0,12){\line(1,0){9}}
\put(0,9){\line(1,0){9}}
\put(0,6){\line(1,0){6}}
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){6}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){12}}
\put(9,12){\line(0,-1){3}}
\end{picture}
}





\def\sYtt{                 %33
\begin{picture}(9,6) 
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){9}}
\put(0,0){\line(1,0){9}}
\put(0,6){\line(0,-1){6}}
\put(3,6){\line(0,-1){6}}
\put(6,6){\line(0,-1){6}}
\put(9,6){\line(0,-1){6}}
\end{picture}
}



\def\sYttj{                 %331
\begin{picture}(9,9) 
\put(0,9){\line(1,0){9}}
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){9}}
\put(0,0){\line(1,0){3}}
\put(0,9){\line(0,-1){9}}
\put(3,9){\line(0,-1){9}}
\put(6,9){\line(0,-1){6}}
\put(9,9){\line(0,-1){6}}
\end{picture}
}


\def\sYttjj{                 %3311
\begin{picture}(9,12) 
\put(0,12){\line(1,0){9}}
\put(0,9){\line(1,0){9}}
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){3}}
\put(0,0){\line(1,0){3}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){6}}
\put(9,12){\line(0,-1){6}}
\end{picture}
}



\def\sYttd{                 %332
\begin{picture}(9,9) 
\put(0,9){\line(1,0){9}}
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){9}}
\put(0,0){\line(1,0){6}}
\put(0,9){\line(0,-1){9}}
\put(3,9){\line(0,-1){9}}
\put(6,9){\line(0,-1){9}}
\put(9,9){\line(0,-1){6}}
\end{picture}
}


\def\sYttdj{                 %3321
\begin{picture}(9,12) 
\put(0,12){\line(1,0){9}}
\put(0,9){\line(1,0){9}}
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){3}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){9}}
\put(9,12){\line(0,-1){6}}
\end{picture}
}


\def\sYttdd{                 %3322
\begin{picture}(9,12) 
\put(0,12){\line(1,0){9}}
\put(0,9){\line(1,0){9}}
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){6}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){12}}
\put(9,12){\line(0,-1){6}}
\end{picture}
}



\def\sYttt{                 %333
\begin{picture}(9,9) 
\put(0,9){\line(1,0){9}}
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){9}}
\put(0,0){\line(1,0){9}}
\put(0,9){\line(0,-1){9}}
\put(3,9){\line(0,-1){9}}
\put(6,9){\line(0,-1){9}}
\put(9,9){\line(0,-1){9}}
\end{picture}
}


\def\sYtttj{                 %3331
\begin{picture}(9,12) 
\put(0,12){\line(1,0){9}}
\put(0,9){\line(1,0){9}}
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){9}}
\put(0,0){\line(1,0){3}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){9}}
\put(9,12){\line(0,-1){9}}
\end{picture}
}


\def\sYtttd{                 %3332
\begin{picture}(9,12) 
\put(0,12){\line(1,0){9}}
\put(0,9){\line(1,0){9}}
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){9}}
\put(0,0){\line(1,0){6}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){12}}
\put(9,12){\line(0,-1){9}}
\end{picture}
}



\def\sYtttt{                 %3333
\begin{picture}(9,12) 
\put(0,12){\line(1,0){9}}
\put(0,9){\line(1,0){9}}
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){9}}
\put(0,0){\line(1,0){9}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){12}}
\put(9,12){\line(0,-1){12}}
\end{picture}
}



\def\sYc{                 %4
\begin{picture}(12,3) 
\put(0,3){\line(1,0){12}}
\put(0,0){\line(1,0){12}}
\put(0,3){\line(0,-1){3}}
\put(3,3){\line(0,-1){3}}
\put(6,3){\line(0,-1){3}}
\put(9,3){\line(0,-1){3}}
\put(12,3){\line(0,-1){3}}
\end{picture}
}



\def\sYcj{                 %41
\begin{picture}(12,6) 
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){12}}
\put(0,0){\line(1,0){3}}
\put(0,6){\line(0,-1){6}}
\put(3,6){\line(0,-1){6}}
\put(6,6){\line(0,-1){3}}
\put(9,6){\line(0,-1){3}}
\put(12,6){\line(0,-1){3}}
\end{picture}
}



\def\sYcjj{                 %411
\begin{picture}(12,9) 
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){3}}
\put(0,0){\line(1,0){3}}
\put(0,9){\line(0,-1){9}}
\put(3,9){\line(0,-1){9}}
\put(6,9){\line(0,-1){3}}
\put(9,9){\line(0,-1){3}}
\put(12,9){\line(0,-1){3}}
\end{picture}
}


\def\sYcjjj{                 %4111
\begin{picture}(12,12) 
\put(0,12){\line(1,0){12}}
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){3}}
\put(0,3){\line(1,0){3}}
\put(0,0){\line(1,0){3}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){3}}
\put(9,12){\line(0,-1){3}}
\put(12,12){\line(0,-1){3}}
\end{picture}
}




\def\sYcd{                 %42
\begin{picture}(12,6) 
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){12}}
\put(0,0){\line(1,0){6}}
\put(0,6){\line(0,-1){6}}
\put(3,6){\line(0,-1){6}}
\put(6,6){\line(0,-1){6}}
\put(9,6){\line(0,-1){3}}
\put(12,6){\line(0,-1){3}}
\end{picture}
}



\def\sYcdj{                 %421
\begin{picture}(12,9) 
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){3}}
\put(0,9){\line(0,-1){9}}
\put(3,9){\line(0,-1){9}}
\put(6,9){\line(0,-1){6}}
\put(9,9){\line(0,-1){3}}
\put(12,9){\line(0,-1){3}}
\end{picture}
}


\def\sYcdjj{                 %4211
\begin{picture}(12,12) 
\put(0,12){\line(1,0){12}}
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){6}}
\put(0,3){\line(1,0){3}}
\put(0,0){\line(1,0){3}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){6}}
\put(9,12){\line(0,-1){3}}
\put(12,12){\line(0,-1){3}}
\end{picture}
}



\def\sYcdd{                 %422
\begin{picture}(12,9) 
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){6}}
\put(0,9){\line(0,-1){9}}
\put(3,9){\line(0,-1){9}}
\put(6,9){\line(0,-1){9}}
\put(9,9){\line(0,-1){3}}
\put(12,9){\line(0,-1){3}}
\end{picture}
}


\def\sYcddj{                 %4221
 \begin{picture}(12,12) 
\put(0,12){\line(1,0){12}}
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){6}}
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){3}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){9}}
\put(9,12){\line(0,-1){3}}
\put(12,12){\line(0,-1){3}}
\end{picture}
}


\def\sYcddd{                 %4222
\begin{picture}(12,12) 
\put(0,12){\line(1,0){12}}
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){6}}
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){6}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){12}}
\put(9,12){\line(0,-1){3}}
\put(12,12){\line(0,-1){3}}
\end{picture}
}





\def\sYct{                 %43
\begin{picture}(12,6) 
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){12}}
\put(0,0){\line(1,0){9}}
\put(0,6){\line(0,-1){6}}
\put(3,6){\line(0,-1){6}}
\put(6,6){\line(0,-1){6}}
\put(9,6){\line(0,-1){6}}
\put(12,6){\line(0,-1){3}}
\end{picture}
}



\def\sYctj{                 %431
\begin{picture}(12,9) 
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){9}}
\put(0,0){\line(1,0){3}}
\put(0,9){\line(0,-1){9}}
\put(3,9){\line(0,-1){9}}
\put(6,9){\line(0,-1){6}}
\put(9,9){\line(0,-1){6}}
\put(12,9){\line(0,-1){3}}
\end{picture}
}


\def\sYctjj{                 %4311
\begin{picture}(12,12) 
\put(0,12){\line(1,0){12}}
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){3}}
\put(0,0){\line(1,0){3}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){6}}
\put(9,12){\line(0,-1){6}}
\put(12,12){\line(0,-1){3}}
\end{picture}
}



\def\sYctd{                 %432
\begin{picture}(12,9) 
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){9}}
\put(0,0){\line(1,0){6}}
\put(0,9){\line(0,-1){9}}
\put(3,9){\line(0,-1){9}}
\put(6,9){\line(0,-1){9}}
\put(9,9){\line(0,-1){6}}
\put(12,9){\line(0,-1){3}}
\end{picture}
}


\def\sYctdj{                 %4321
 \begin{picture}(12,12) 
\put(0,12){\line(1,0){12}}
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){3}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){9}}
\put(9,12){\line(0,-1){6}}
\put(12,12){\line(0,-1){3}}
\end{picture}
}


\def\sYctdd{                 %4322
\begin{picture}(12,12) 
\put(0,12){\line(1,0){12}}
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){6}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){12}}
\put(9,12){\line(0,-1){6}}
\put(12,12){\line(0,-1){3}}
\end{picture}
}


\def\sYctt{                 %433
\begin{picture}(12,9) 
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){9}}
\put(0,0){\line(1,0){9}}
\put(0,9){\line(0,-1){9}}
\put(3,9){\line(0,-1){9}}
\put(6,9){\line(0,-1){9}}
\put(9,9){\line(0,-1){9}}
\put(12,9){\line(0,-1){3}}
\end{picture}
}


\def\sYcttj{                 %4331
 \begin{picture}(12,12) 
\put(0,12){\line(1,0){12}}
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){9}}
\put(0,0){\line(1,0){3}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){9}}
\put(9,12){\line(0,-1){9}}
\put(12,12){\line(0,-1){3}}
\end{picture}
}


\def\sYcttd{                 %4332
 \begin{picture}(12,12) 
\put(0,12){\line(1,0){12}}
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){9}}
\put(0,0){\line(1,0){6}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){12}}
\put(9,12){\line(0,-1){9}}
\put(12,12){\line(0,-1){3}}
\end{picture}
}


\def\sYcttt{                 %4333
 \begin{picture}(12,12) 
\put(0,12){\line(1,0){12}}
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){9}}
\put(0,3){\line(1,0){9}}
\put(0,0){\line(1,0){9}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){12}}
\put(9,12){\line(0,-1){12}}
\put(12,12){\line(0,-1){3}}
\end{picture}
}


\def\sYcc{                 %44
\begin{picture}(12,6) 
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){12}}
\put(0,0){\line(1,0){12}}
\put(0,6){\line(0,-1){6}}
\put(3,6){\line(0,-1){6}}
\put(6,6){\line(0,-1){6}}
\put(9,6){\line(0,-1){6}}
\put(12,6){\line(0,-1){6}}
\end{picture}
}


\def\sYccj{                 %441
\begin{picture}(12,9) 
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){12}}
\put(0,0){\line(1,0){3}}
\put(0,9){\line(0,-1){9}}
\put(3,9){\line(0,-1){9}}
\put(6,9){\line(0,-1){6}}
\put(9,9){\line(0,-1){6}}
\put(12,9){\line(0,-1){6}}
\end{picture}
}


\def\sYccjj{                 %4411
\begin{picture}(12,12) 
\put(0,12){\line(1,0){12}}
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){3}}
\put(0,0){\line(1,0){3}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){6}}
\put(9,12){\line(0,-1){6}}
\put(12,12){\line(0,-1){6}}
\end{picture}
}



\def\sYccd{                 %442
\begin{picture}(12,9) 
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){12}}
\put(0,0){\line(1,0){6}}
\put(0,9){\line(0,-1){9}}
\put(3,9){\line(0,-1){9}}
\put(6,9){\line(0,-1){9}}
\put(9,9){\line(0,-1){6}}
\put(12,9){\line(0,-1){6}}
\end{picture}
}


\def\sYccdj{                 %4421
 \begin{picture}(12,12) 
\put(0,12){\line(1,0){12}}
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){3}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){9}}
\put(9,12){\line(0,-1){6}}
\put(12,12){\line(0,-1){6}}
\end{picture}
}


\def\sYccdd{                 %4422
 \begin{picture}(12,12) 
\put(0,12){\line(1,0){12}}
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){6}}
\put(0,0){\line(1,0){6}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){12}}
\put(9,12){\line(0,-1){6}}
\put(12,12){\line(0,-1){6}}
\end{picture}
}


\def\sYcct{                 %443
\begin{picture}(12,9) 
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){12}}
\put(0,0){\line(1,0){9}}
\put(0,9){\line(0,-1){9}}
\put(3,9){\line(0,-1){9}}
\put(6,9){\line(0,-1){9}}
\put(9,9){\line(0,-1){9}}
\put(12,9){\line(0,-1){6}}
\end{picture}
}


\def\sYcctj{                 %4431
 \begin{picture}(12,12) 
\put(0,12){\line(1,0){12}}
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){9}}
\put(0,0){\line(1,0){3}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){9}}
\put(9,12){\line(0,-1){9}}
\put(12,12){\line(0,-1){6}}
\end{picture}
}


\def\sYcctd{                 %4432
 \begin{picture}(12,12) 
\put(0,12){\line(1,0){12}}
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){9}}
\put(0,0){\line(1,0){6}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){12}}
\put(9,12){\line(0,-1){9}}
\put(12,12){\line(0,-1){6}}
\end{picture}
}


\def\sYcctt{                 %4433
 \begin{picture}(12,12) 
\put(0,12){\line(1,0){12}}
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){9}}
\put(0,0){\line(1,0){9}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){12}}
\put(9,12){\line(0,-1){12}}
\put(12,12){\line(0,-1){6}}
\end{picture}
}



\def\sYccc{                 %444
\begin{picture}(12,9) 
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){12}}
\put(0,0){\line(1,0){12}}
\put(0,9){\line(0,-1){9}}
\put(3,9){\line(0,-1){9}}
\put(6,9){\line(0,-1){9}}
\put(9,9){\line(0,-1){9}}
\put(12,9){\line(0,-1){9}}
\end{picture}
}



\def\sYcccj{                 %4441
 \begin{picture}(12,12) 
\put(0,12){\line(1,0){12}}
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){12}}
\put(0,0){\line(1,0){3}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){9}}
\put(9,12){\line(0,-1){9}}
\put(12,12){\line(0,-1){9}}
\end{picture}
}



\def\sYcccd{                 %4442
 \begin{picture}(12,12) 
\put(0,12){\line(1,0){12}}
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){12}}
\put(0,0){\line(1,0){6}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){12}}
\put(9,12){\line(0,-1){9}}
\put(12,12){\line(0,-1){9}}
\end{picture}
}



\def\sYccct{                 %4443
 \begin{picture}(12,12) 
\put(0,12){\line(1,0){12}}
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){12}}
\put(0,0){\line(1,0){9}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){12}}
\put(9,12){\line(0,-1){12}}
\put(12,12){\line(0,-1){9}}
\end{picture}
}



\def\sYcccc{                 %4444
 \begin{picture}(12,12) 
\put(0,12){\line(1,0){12}}
\put(0,9){\line(1,0){12}}
\put(0,6){\line(1,0){12}}
\put(0,3){\line(1,0){12}}
\put(0,0){\line(1,0){12}}
\put(0,12){\line(0,-1){12}}
\put(3,12){\line(0,-1){12}}
\put(6,12){\line(0,-1){12}}
\put(9,12){\line(0,-1){12}}
\put(12,12){\line(0,-1){12}}
\end{picture}
}



